Safe Disassociation of Set-Valued Datasets

Disassociation introduced by Terrovitis et al. is a bucketization based anonimyzation technique that divides a set-valued dataset into several clusters to hide the link between individuals and their complete set of items. It increases the utility of the anonymized dataset, but on the other side, it raises many privacy concerns, one in particular, is when the items are tightly coupled to form what is called, a cover problem. In this paper, we present safe disassociation, a technique that relies on partial-suppression, to overcome the aforementioned privacy breach encountered when disassociating set-valued datasets. Safe disassociation allows the $k^m$-anonymity privacy constraint to be extended to a bucketized dataset and copes with the cover problem. We describe our algorithm that achieves the safe disassociation and we provide a set of experiments to demonstrate its efficiency.

==> resultsgraph.tex <==
Dataset,DatasetSize,distinct individuals,k,m,MaxClusterSize,TermOccurences,Loss Metric,percOccurencesLost,RC count,RC partial Supp ,RC full Suppress,perc RC affected,RE,RE Safe Diss,percREincrease,RunTime msec
BMS1,149639,59602,3,2,10,88814,4905,5.52277794,6774,905,287,17.59669324,106653.1732,107044.7124,0.367114446,
BMS1,149639,59602,3,2,20,94941,9126,9.612285525,5103,957,663,31.74603175,105541.2859,106193.4778,0.617949484,
BMS1,149639,59602,3,2,30,98743,11631,11.77906282,4695,933,954,40.19169329,104430.1494,105173.9537,0.712250522,
BMS1,149639,59602,3,2,40,101339,14430,14.2393353,4507,896,1139,45.1519858,104406.2819,111199.2445,6.506277685,
BMS1,149639,59602,3,2,50,103385,12515,12.1052377,4491,871,1353,49.52126475,104143.6567,104867.0067,0.694569448,
BMS1,149639,59602,3,2,60,104867,12396,11.82068716,4467,853,1506,52.80949183,104006.1643,104789.229,0.752902262,
,,,,,,,,,,,,,,,,
BMS2,358278,77512,3,2,10,132649,15719,11.85007049,10042,1770,891,26.49870544,1437468.337,1438746.764,0.088935995,
BMS2,358278,77512,3,2,20,148229,26567,17.92294355,9509,1679,2126,40.01472289,1437388.542,1438690.183,0.090555952,
BMS2,358278,77512,3,2,30,156525,30806,19.68120109,9699,1538,3037,47.16981132,1437434.212,1438669.754,0.085954689,
BMS2,358278,77512,3,2,40,163007,30646,18.80041961,10008,1445,3715,51.558753,1437462.515,1438556.924,0.076134767,
BMS2,358278,77512,3,2,50,167519,30825,18.40089781,10184,1362,4174,54.35978005,1437442.923,1438437.705,0.069204923,
BMS2,358278,77512,3,2,60,171956,32441,18.86587267,10438,1291,4635,56.77332822,1437481,1438438.8,0.066630452,
,,,,,,,,,,,,,,,,
BMS1,10000,,,,,,,,,,,,,,,11
BMS1,30000,,,,,,,,,,,,,,,30
BMS1,50000,,,,,,,,,,,,,,,59
BMS1,80000,,,,,,,,,,,,,,,85
BMS1,100000,,,,,,,,,,,,,,,94
BMS1,149639,,,,,,,,,,,,,,,118
BMS2,358278,,,,,,,,,,,,,,,136
,,,,,,,,,,,,,,,,
BMS1,149639,59602,2,2,30,111959,24089,21.51591207,7458,1020,2466,46.74175382,,,,
BMS1,149639,59602,3,2,30,98743,11631,11.77906282,4695,933,954,40.19169329,,,,
BMS1,149639,59602,4,2,30,90733,5959,6.567621483,3455,807,400,34.93487699,,,,
BMS1,149639,59602,5,2,30,85149,3292,3.866164018,2835,715,194,32.06349206,,,,
BMS1,149639,59602,6,2,30,81439,2517,3.090656811,2503,642,116,30.28365961,,,,
BMS1,149639,59602,2,2,30,111959,24089,21.51591207,7458,1020,2466,46.74175382,,,,
BMS1,149639,59602,2,3,30,111959,26230,23.42821926,7454,1013,2470,46.72658975,,,,
BMS1,149639,59602,2,4,30,111959,26395,23.57559464,7450,1013,2466,46.69798658,,,,
BMS1,149639,59602,2,5,30,111959,26395,23.57559464,7450,1013,2466,46.69798658,,,,
BMS1,149639,59602,2,6,30,111959,26395,23.57559464,7450,1013,2466,46.69798658,,,,
BMS1,149639,59602,4,4,30,90733,6634,7.311562497,3463,801,410,34.96967947,,,,
,,,,,,,,,,,,,,,,
BMS2,358278,77512,2,2,30,191969,63605,33.13295376,18210,1467,8859,56.70510708,,,,
BMS2,358278,77512,3,2,30,156525,30806,19.68120109,9699,1538,3037,47.16981132,,,,
BMS2,358278,77512,4,2,30,138720,19271,13.89201269,6549,1392,1335,41.63994503,,,,
BMS2,358278,77512,5,2,30,126904,12172,9.591502238,5024,1289,712,39.82882166,,,,
BMS2,358278,77512,6,2,30,118039,9591,8.125280628,4131,1168,434,38.77995643,,,,
BMS2,358278,77512,2,2,30,191969,63605,33.13295376,18210,1467,8859,56.70510708,,,,
BMS2,358278,77512,2,3,30,191969,67788,35.31195141,18264,1462,8879,56.6195795,,,,
BMS2,358278,77512,2,4,30,191969,67834,35.33591361,18265,1462,8880,56.62195456,,,,
BMS2,358278,77512,2,5,30,191969,67837,35.33747636,18265,1462,8881,56.62742951,,,,
BMS2,358278,77512,2,6,30,191969,67837,35.33747636,18265,1462,8881,56.62742951,,,,

